StartupBR: Higher Education's Influence on Social Networks and Entrepreneurship in Brazil

Developing and middle-income countries increasingly empha-size higher education and entrepreneurship in their long-term develop-ment strategy. Our work focuses on the influence of higher education institutions (HEIs) on startup ecosystems in Brazil, an emerging economy. First, we describe regional variability in entrepreneurial network characteristics. Then we examine the influence of elite HEIs in economic hubs on entrepreneur networks. Second, we investigate the influence ofthe academic trajectories of startup founders, including their courses of study and HEIs of origin, on the fundraising capacity of startups. Given the growing capability of social media databases such as Crunchbase and LinkedIn to provide startup and individual-level data, we draw on computational methods to mine data for social network analysis. We find that HEI quality and the maturity of the ecosystem influence startup success. Our network analysis illustrates that elite HEIs have powerful influences on local entrepreneur ecosystems. Surprisingly, while the most nationally prestigious HEIs in the South and Southeast have the longest geographical reach, their network influence still remains local.

==> backup.tex <==
\begin{itemize}
    \item \textbf{Crunchbase:} is a database that contains information about companies in the world, increasingly used in recent years for both academic and commercial purposes.   \cite{crunch12,Dalle2017}. Crunchbase is a partially crowd-sourced database, updated daily, and contains data on companies, funders, and staff \textcolor{green}{(Dal, des Beston, Menon, 2017) \cite{Dalle2017}}. To obtain Crunchbase data, we acquired a commercial license which enabled unlimited access in addition to advanced search functions. In this study, we obtain all available data of Brazilian companies up to August 26, 2018, with information from 3,375 companies spread throughout Brazil. The primary data collected includes company name; URL to the LinkedIn profile; date of statup founding; company type (or category); the total of investments received; and headquarters location.
    
    Crunchbase is unique in terms of its linkability to other data sources, for example, Twitter (Tata et al., 2016, Tata et al. 2017) and LinkedIn \textcolor{green}{(Nuscheler, 2016 in Dal, des Beston, and Menon, 2017)\cite{Dalle2017}}. Given that potential, we linked Crunchbase with LinkedIn, to examine characteristics of the startup founders, their universities where they studied, and their social networks.

    \item \textbf{LinkedIn:} is a popular social network of professional contacts. LinkedIn provided the educational information of the startup founders. With the LinkedIn profile URL, which we obtained through Crunchbase, we collected the profiles of employees that held titles such as CEO, owner, and founder. In the end, this yielded 1,177 profiles and the main data collected were: degree type (e.g., M.Sc., or Ph.D.); degree area (e.g., Sociology, or Computer Science); graduation year; and the name of the alma mater. Multiple degrees for the same profile were common. We collected all the information described on the LinkedIn profile.
    
    \item \textbf{IGC:} The National Institute of Educational Studies and Research of Brazil (INEP\footnote{http://portal.inep.gov.br.}) annually performs the Census of Higher Education (CENSUP\footnote{http://sistemascensosuperior.inep.gov.br/censosuperior_2018/}). The census provides data for the General Index of Courses (IGC\footnote{http://inep.gov.br/en/indice-geral-de-cursos-igc-}), the official quality indicator for Brazilian HEIs. We draw on the latest released data, the 2016 INEP website data. Our data refer to the 2016 INEP data, and we use the IGC index when available for all HEIs in our dataset.
    `
\end{itemize}
